Three Attacks on Proof-of-Stake Ethereum

Recently, two attacks were presented against Proof-of-Stake (PoS) Ethereum: one where short-range reorganizations of the underlying consensus chain are used to increase individual validators' profits and delay consensus decisions, and one where adversarial network delay is leveraged to stall consensus decisions indefinitely. We provide refined variants of these attacks, considerably relaxing the requirements on adversarial stake and network timing, and thus rendering the attacks more severe. Combining techniques from both refined attacks, we obtain a third attack which allows an adversary with vanishingly small fraction of stake and no control over network message propagation (assuming instead probabilistic message propagation) to cause even long-range consensus chain reorganizations. Honest-but-rational or ideologically motivated validators could use this attack to increase their profits or stall the protocol, threatening incentive alignment and security of PoS Ethereum. The attack can also lead to destabilization of consensus from congestion in vote processing.

==> figures/exante-reorg/ex-ante-reorg-timing.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/exante-reorg/ex-ante-reorg-timing.png}
    \captionsetup{singlelinecheck=off}
    \caption[]{An ideal ex-ante reorg attack is described as follows:
\begin{enumerate}[label={--}]
\item Slot $n$: The block \& attestations are produced.
\item Slot $n+1$: Attacker controls the proposer and a single attester. It produces a block \& attestation, but does not publish it until slot $n+2$. Honest attesters vote for the publicly known head block at slot $n$
\item Slot $n+2$: The proposer produces a block on top of the publicly known head block at slot $n$. At the same time, the attacker releases block $n+1$ and its attestation to block $n+1$, such that at least half of the honest attesters in this slot receive these messages before block $n+2$. Hence, at least half of the honest attesters produce attestations for the attacker's block $n+1$.
\item Slot $n+3$: The proposer sees block $n+1$ as the head block and produces its block on top of it. Block $n+2$ is orphaned.
\end{enumerate}
}
    \label{fig:exante-reorg-timing}
\end{figure}
